A Wait-Free Universal Construct for Large Objects

Concurrency has been a subject of study for more than 50 years. Still, many developers struggle to adapt their sequential code to be accessed concurrently. This need has pushed for generic solutions and specific concurrent data structures. Wait-free universal constructs are attractive as they can turn a sequential implementation of any object into an equivalent, yet concurrent and wait-free, implementation. While highly relevant from a research perspective, these techniques are of limited practical use when the underlying object or data structure is sizable. The copy operation can consume much of the CPU's resources and significantly degrade performance. To overcome this limitation, we have designed CX, a multi-instance-based wait-free universal construct that substantially reduces the amount of copy operations. The construct maintains a bounded number of instances of the object that can potentially be brought up to date. We applied CX to several sequential implementations of data structures, including STL implementations, and compared them with existing wait-free constructs. Our evaluation shows that CX performs significantly better in most experiments, and can even rival with hand-written lock-free and wait-free data structures, simultaneously providing wait-free progress, safe memory reclamation and high reader scalability.

==> 5-support.tex <==
%!TEX root = 0-main.tex

\section{Programming Language Support}
\label{sec:support}

The \CX universal construct provides concurrent wait-free progress to any user-developed sequential object that it encapsulates. 
This object can be a single data structure, or it can contain multiple references to different data structures or objects.
Applications that usually require a specific data structure, or complex filtering of the data, can take advantage of \CX's flexibility.
Also, \CX allows users to define dynamic functions, as long as they involve data accessible from the encapsulated object.

In algorithm~\ref{alg:cxset} we present how \CX can be used to transform \texttt{std::set} sequential implementation into a concurrent set with wait-free insertion, deletions and lookups, when $maxObjs=2 \times maxThreads$.
In case the application does not require the resilience provided by the wait-free progress, it is possible to configure \CX to use at most $maxObjs$ where $maxObjs<2 \times maxThreads$.
This configuration implies that the \texttt{applyUpdate()} method will no longer be wait-free, but instead blocking because there will not be enough \texttt{Combined} instances available to guarantee progress.

On the other hand, the \texttt{applyRead()} method will continue to have wait-free progress. 
This progress is guaranteed because only two scenarios can occur.
In the most common scenario, the read operation is able to acquire the shared lock on the $curComb$ combined instance and execute its operation.
Otherwise, if the read operation fails to acquire the shared lock, this means that a write operation transitioned $curComb$.
Once the read operation is added to the wait-free queue, after a maximum of $maxThreads$ failed attempts to acquire the shared lock on $curComb$, the result of the read operation is available on the wait-free queue, executed by a writer helper thread.

Another important detail is that memory reclamation continues to be wait-free. 
In the event of a thread failure, it may happen that at most two copies of the object can not be reclaimed, and a maximum of 2000 nodes can remain unclaimed.
We present in \S\ref{sec:evaluation} an experiment with measurements of throughput and maximum memory usage for different $maxObjs$ configurations.

\begin{algorithm}[ht]
\caption{Making a wait-free set with CX and \texttt{std::set}}
\label{alg:cxset}
\begin{lstlisting}
template<typename K> class WaitFreeSet {
  const int maxThreads;
  const int maxObjs;
  CX<std::set<K>> cxset {
      new std::set<K>, maxThreads, maxObjs};
public:
  WaitFreeSet(int maxThreads=64, int maxObjs=64*2) : 
      maxThreads{maxThreads}, maxObjs{maxObjs} { }

bool add(K key) { (*@\hfill@*) // This method is wait-free
  return cxset.applyUpdate( [=] (auto* set) {
    // Example of a dynamic function
    if (set->find(key) == set->end()) {
      set->insert(key);
      return true;
    }
    return false;
  });
}

bool remove(K key) { (*@\hfill@*) // This method is wait-free
  return cxset.applyUpdate( [=] (auto* set) {
    auto iter = set->find(key);
    if (iter == set->end()) return false;
    set->erase(iter);
    return true;
  });
}

bool contains(K key) { (*@\hfill@*) // This method is wait-free
  return cxset.applyRead( [=] (auto* set) {
    return (set->find(key) != set->end());
  });
}
};	

int main(void) {
  WaitFreeSet<int> wfset;  (*@\hfill@*) // Instanciate a wait-free set
  int key = 33;
  wfset.add(key); (*@\hfill@*) // Insert key 33
  assert(wfset.contains(key));
  wfset.remove(key); (*@\hfill@*) // Remove key 33
  assert(!wfset.contains(key));
  return 0;
}
\end{lstlisting}
\end{algorithm}

Despite its simplicity in adapting sequential implementations to wait-freedom, near future functionality in the C++ language, such as \emph{metaclasses}~\cite{metaclass}, is likely to make it even simpler, by providing the syntactic sugar needed to automatically create a class with exactly the same methods and signatures as the sequential implementation, but wrapped in calls to \texttt{applyRead()} or \texttt{applyUpdate()}, depending on whether the methods are \texttt{const} or not, respectively.
With metaclasses, the user can simply declare the type with a template of the sequential data structure (for example, \texttt{CX<SequentialSet>~wfset;}) and obtain an instance whose methods are wait-free.
